Dual Structure-Aware Image Filterings for Semi-supervised Medical Image Segmentation

Semi-supervised image segmentation has attracted great attention recently. The key is how to leverage unlabeled images in the training process. Most methods maintain consistent predictions of the unlabeled images under variations (e.g., adding noise/perturbations, or creating alternative versions) in the image and/or model level. In most image-level variation, medical images often have prior structure information, which has not been well explored. In this paper, we propose novel dual structure-aware image filterings (DSAIF) as the image-level variations for semi-supervised medical image segmentation. Motivated by connected filtering that simplifies image via filtering in structure-aware tree-based image representation, we resort to the dual contrast invariant Max-tree and Min-tree representation. Specifically, we propose a novel connected filtering that removes topologically equivalent nodes (i.e. connected components) having no siblings in the Max/Min-tree. This results in two filtered images preserving topologically critical structure. Applying the proposed DSAIF to mutually supervised networks decreases the consensus of their erroneous predictions on unlabeled images. This helps to alleviate the confirmation bias issue of overfitting to noisy pseudo labels of unlabeled images, and thus effectively improves the segmentation performance. Extensive experimental results on three benchmark datasets demonstrate that the proposed method significantly/consistently outperforms some state-of-the-art methods. The source codes will be publicly available.

==> algorithm/tree_construction_suppl0.tex <==
\begin{algorithm}
    \SetAlgoLined 
	\caption{Min-tree and Max-tree construction.}
        \label{alg:Min-MAX-tree-construction}
        \tcp{$\mathcal{R}$ : set of sorted pixels }
        \tcp{$N$ : total number of pixels}
        \tcp{$p, q, n, x$ : pixels}
        \tcp{$\mathcal{N}$ : neighbors}
        \tcp{$parent$ : image of parenthood}
        \tcp{$zpar$ : temporary parenthood}
        \tcp{$area$ : area of region}
	\KwIn{An image $f$.}
	\KwOut{Max-tree(Min-tree) of image $f$, areas of nodes.}

        \SetKwFunction{FROOT}{FIND\_ROOT}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\FROOT{$x$}}{
            \Begin{ 
            \eIf{$zpar(x)=x$}{\textbf{return} $x$ }{$zpar(x) \leftarrow \FROOT{zpar(x)}$\;
            \textbf{return} $zpar(x)$
            }
            }
         }


        \SetKwFunction{UNION}{UNION\_FIND}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\UNION{$\mathcal{R}$}}{
            \Begin{ 
            \For{ $p \in \mathcal{R}$}
            {$zpar(p) \leftarrow \text{undef}$\;
            $area(p) \leftarrow 0$ \;
            }
            
            \For{ $i = N-1:0$}
            {
            $p \leftarrow \mathcal{R}[i]$\;
            $parent(p) \leftarrow p$\;
            $zpar(p) \leftarrow p$ \;
            $area(p) \leftarrow 1$ \;
                \For{ $n \in \mathcal{N}(p) \cap zpar(n) \neq undef$}
                {
                    $r \leftarrow \FROOT{n}$\;             
                    \If{$r \neq p$}
                    {
                    $parent(r) \leftarrow p$ \;
                    $zpar(r) \leftarrow p$\;
                    $area(p) \leftarrow area(p)+area(r)$\;
                    }
                }
            
            }
            \textbf{return} $parent, area$
            }
      }

        \SetKwFunction{CANONIZE}{CANONIZE\_TREE}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\CANONIZE{$f$, $\mathcal{R}$, $parent$}}{
            \Begin{ 
            \For{ $i = 0:N-1 $}{
            $p \leftarrow \mathcal{R}[i]$\;
            $q \leftarrow parent(p)$\; 
            \If{$f(parent(q)) = f(q)$}{$parent(p) \leftarrow parent(q)$ \;}
            
            }
            \textbf{return} $parent$
            }
        }

        % \SetKwFunction{MINMAX}{COMPUTE\_MIN\_MAX\_TREE}
        % \SetKwProg{Fn}{Function}{:}{}
        % \Fn{\MINMAX{$f$}}{
        % \Begin{
        % $\mathcal{R} \leftarrow \FuncSty{SORT\_MONOTONE}(f)$ \;
        % $parent,area \leftarrow$ \UNION{$\mathcal{R}$}\;
        % $parent \leftarrow$ \CANONIZE{f, $\mathcal{R}$, parent}\;
        % \textbf{return} $parent, area$
        % }
        % }
\end{algorithm}

==> table/ACDC-new.tex <==
\begin{table}
  \centering
  \caption{Quantitative segmentation results on the ACDC dataset~\cite{bernard2018deep}.~\dag~represents the reproduced results based on the open-sourced implementation.}
  \label{tab:ACDC}
  \setlength{\tabcolsep}{1mm}
    % \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{clcccc}
    \hline
    L/U &Method &DSC$\uparrow$ &JAC$\uparrow$ &95HD$\downarrow$ &ASD$\downarrow$ \\
    \hline
    70/0 &U-Net\dag &91.20 &84.25 &2.52 &0.68 \\
    \hline
    7/0   &U-Net\dag &79.65 &68.57 &8.32 &2.51 \\
    \hline
     \multirow{7}*{7/63} &UA-MT~\cite{yu2019uncertainty}  &81.58 &70.48&12.35&3.62\\
     &URPC~\cite{luo2021efficient}     &81.77 &70.85 & 5.04& 1.41\\
     &SS-Net~\cite{wu2022exploring}   &86.78      &77.67   &6.07    &1.40\\ 
     &SALCC~\cite{liu2022semi}       &82.49  &-  &-  &1.05 \\
     &MC-Net$+$~\cite{wu2022mutual}    &87.10 &78.06 &6.68 &2.00\\
     \cline{2-6}
     &CPS~\cite{chen2021semi}\dag   &88.65\scriptsize(0.00)   &80.13\scriptsize(0.00)   &5.27\scriptsize(0.00)   & 2.17\scriptsize(0.00)\\
     &Ours  &\textbf{89.13}\scriptsize(0.00) &\textbf{80.93}\scriptsize(0.00) &\textbf{3.73}\scriptsize(0.00) &\textbf{0.97}\scriptsize(0.00) \\
    \hline
    14/0 &U-Net\dag &83.69 &73.87 &8.58 &2.42 \\
    \hline
    \multirow{6}*{14/56} &UA-MT~\cite{yu2019uncertainty}  &85.87 &76.78 &5.06 &1.54\\
      &URPC~\cite{luo2021efficient}    & 85.07 &75.61  &6.26  &1.77 \\
      &SALCC~\cite{liu2022semi}\dag      &85.68  &75.88  &4.55  &0.91 \\
      &MC-Net$+$~\cite{wu2022mutual} &88.51 &80.19 &5.35 &1.54\\
      \cline{2-6}
    &CPS~\cite{chen2021semi}\dag     &89.54\scriptsize(0.00)  &81.86\scriptsize(0.00)  &3.69\scriptsize(0.00)  &0.98\scriptsize(0.00) \\
     &Ours &\textbf{90.00}\scriptsize(0.00) &\textbf{82.38}\scriptsize(0.00) &\textbf{2.56}\scriptsize(0.00) &\textbf{0.79}\scriptsize(0.00) \\
    \hline
  \end{tabular} 
  % }
\end{table}

==> table/ACDC.tex <==
\begin{table*}[]
  \centering
  \caption{Quantitative segmentation results on the ACDC dataset~\cite{bernard2018deep}.~\dag~represents the reproduced results based on the open-sourced implementation.}
  \label{tab:ACDC}
  % \setlength{\tabcolsep}{1mm}
    % \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c}{\#Scans used} &\multicolumn{4}{c}{Metrics} \\
    \cline{2-3} \cline{4-7} 
    &Labeled &Unlabeled &Dice(\%)$\uparrow$ &Jaccard(\%)$\uparrow$ &95HD$\downarrow$ &ASD$\downarrow$ \\
    \hline
    U-Net\dag &70 &0 &91.20 &84.25 &2.52 &0.68 \\
    \hline
    U-Net\dag &7  &0 &79.65 &68.57 &8.32 &2.51 \\
    UA-MT~\cite{yu2019uncertainty}(MICCAI 2019) &7  &63  &81.58 &70.48 &12.35 &3.62\\
    URPC~\cite{luo2021efficient} \scriptsize{(MICCAI'21)} &7 &63     &81.77 &70.85 & 5.04& 1.41\\
    CPS~\cite{chen2021semi}\dag \scriptsize{(CVPR'21) } &7 &63    &88.65   &80.13   &5.27   & 2.17\\
    SS-Net~\cite{wu2022exploring} \scriptsize{(MICCAI'22)}  &7 &63    &86.78      &77.67   &6.07    &1.40\\ 
    SALCC~\cite{liu2022semi} \scriptsize{(MICCAI'22)}  &7 &63      &82.49  &-  &-  &1.05 \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &7 &63     &87.10 &78.06 &6.68 &2.00\\
    Ours &7 &63 &\textbf{89.13} &\textbf{80.93} &\textbf{3.73} &\textbf{0.97} \\
    \hline
    U-Net\dag &14  &0 &83.69 &73.87 &8.58 &2.42 \\
    UA-MT~\cite{yu2019uncertainty}(MICCAI 2019) &14  &56  &85.87 &76.78 &5.06 &1.54\\
    URPC~\cite{luo2021efficient} \scriptsize{(MICCAI'21)} &14  &56     & 85.07 &75.61  &6.26  &1.77 \\
    CPS~\cite{chen2021semi}\dag \scriptsize{(CVPR'21)} &14  &56      &89.54  &81.86  &3.69  &0.98 \\
    SALCC~\cite{liu2022semi}\dag \scriptsize{(MICCAI'22) } &14  &56      &85.68  &75.88  &4.55  &0.91 \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &14  &56 &88.51 &80.19 &5.35 &1.54\\
    Ours &14  &56 &\textbf{90.00} &\textbf{82.38} &\textbf{2.56} &\textbf{0.79} \\
    \hline
  \end{tabular} 
  % }
\end{table*}

==> table/LA.tex <==
\begin{table*}
  \centering
  \caption{Quantitative segmentation results on the LA dataset~\cite{xiong2021global}.~\dag~represents the reproduced results based on the open-sourced implementation.}
  \label{tab:LA}
  % \setlength{\tabcolsep}{1mm}
  % \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c}{\#Scans used} &\multicolumn{4}{c}{Metrics} \\
    \cline{2-3} \cline{4-7} 
    &Labeled &Unlabeled &Dice(\%)$\uparrow$ &Jaccard(\%)$\uparrow$ &95HD$\downarrow$ &ASD$\downarrow$ \\
    \hline
    V-Net\dag &80  &0 &91.82 &84.92 &5.12 &1.71 \\
    \hline
    V-Net\dag &8  &0 &80.75 &69.81 &15.11 &3.61 \\
    UA-MT~\cite{yu2019uncertainty}(MICCAI 2019) &8  &72  &86.28 &76.11 &18.71 &4.63\\
    URPC~\cite{luo2021efficient}(MICCAI 2021) & &     &85.01 &74.36 &15.37 &3.96 \\
    CPS\dag~\cite{chen2021semi} \scriptsize{(CVPR'21)} &8 &72      &87.72   &78.35  &11.77  &3.38 \\
    GBDL~\cite{wang2022rethinking} (CVPR 2022) & &      &88.40   &0.792  &\textbf{5.89}  &\textbf{1.60} \\
    CVRL~\cite{you2022momentum} \scriptsize{(MICCAI'22)} &8 &72      &88.56   &78.89  &8.22  &2.81 \\
    SS-Net~\cite{wu2022exploring} \scriptsize{(MICCAI'22)}  &8 &72    &88.55      &79.62   &\textbf{7.49}   &1.90\\
    SimCVD~\cite{you2022simcvd} \scriptsize{(TMI'22)}  &8 &72      &89.03   &80.34  &8.34 &2.59 \\
    LLRU~\cite{adiga2022leveraging} \scriptsize{(MICCAI'22)}  &8 &72      &86.58  &-  &11.82 &- \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &8 &72 &88.96 &80.25 &7.93 &\textbf{1.86}\\
    Ours &8 &72 &\textbf{89.50} &\textbf{81.13} &8.41 &2.29 \\
    \hline
    V-Net\dag &16  &0 &88.41 &79.43 &10.05 &2.40 \\
    UA-MT~\cite{yu2019uncertainty}(MICCAI 2019) &16  &64  &88.74 &79.94 &8.39 &2.32\\
    URPC~\cite{luo2021efficient}(MICCAI 2021) & &     &88.74 &79.93 &12.73 &3.66 \\
    CPS\dag~\cite{chen2021semi} \scriptsize{(CVPR'21)} &16 &64      &89.69  &81.45  &7.37  &2.24 \\
    GBDL~\cite{wang2022rethinking} (CVPR 2022) & &      &89.4   &0.822  &\textbf{4.03}  &\textbf{1.48} \\
    CVRL~\cite{you2022momentum} \scriptsize{(MICCAI'22)} &16 &64      &90.45   &83.02 &6.56  &1.81 \\
    SimCVD~\cite{you2022simcvd} \scriptsize{(TMI'22)}  &16 &64      &90.85   &83.80  &6.03 &1.86 \\
    LLRU~\cite{adiga2022leveraging} \scriptsize{(MICCAI'22)}  &16 &64      &88.60  &-  &7.61 &- \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &16 &64 &91.07&83.67 &5.84 &1.67\\
    Ours &16 &64 &\textbf{91.32} &\textbf{84.08} &\textbf{5.16} &\textbf{1.62} \\
    \hline
   \end{tabular} 
   % }
\end{table*}

==> table/PROMISE12.tex <==
\begin{table*}
  \centering
  \caption{Quantitative segmentation results on the PROMISE12 dataset~\cite{litjens2014evaluation}. ~\dag~represents the reproduced results based on the open-sourced implementation.}
  \label{tab:PROMISE12}
  % \setlength{\tabcolsep}{1mm}
    % \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c}{\#Scans used} &\multicolumn{4}{c}{Metrics} \\
    \cline{2-3} \cline{4-7} 
    &Labeled &Unlabeled &Dice(\%)$\uparrow$ &Jaccard(\%)$\uparrow$ &95HD$\downarrow$ &ASD$\downarrow$ \\
    \hline
    U-Net\dag &35  &0 &84.63  &73.73  &3.63  &1.27  \\
    \hline
    U-Net\dag &4  &0   &51.72  &39.02  &43.30  &11.81 \\
    UA-MT~\cite{yu2019uncertainty}\dag \scriptsize{(MICCAI'19)} &4 &31 &49.81  &37.52  &74.03  &15.95   \\
    URPC~\cite{luo2021efficient}\dag \scriptsize{(MICCAI'21)} &4 &31     &51.70 &38.30 &75.19 & 22.32 \\
    CPS~\cite{chen2021semi}\dag \scriptsize{(CVPR'21)} &4 &31      &57.10  &44.16  &32.00  &6.38 \\
    SALCC~\cite{liu2022semi}\dag \scriptsize{(MICCAI'22)}  &4 &31      &63.85 &48.07  &40.68  &7.50 \\
    MC-Net$+$~\cite{wu2022mutual}\dag \scriptsize{(MIA'22)} &4 &31    &55.40  &42.01  &21.79  & 5.51 \\
    Ours  &4 &31     &\textbf{78.42} &\textbf{65.36} &\textbf{6.96} &\textbf{2.70} \\
    \hline
    U-Net\dag &7  &0 &65.63  &52.44  &12.36  &2.98  \\
    UA-MT~\cite{yu2019uncertainty} \scriptsize{(MICCAI'19)} &7  &28  &61.55  &-  &-  &13.94 \\
    URPC~\cite{luo2021efficient} \scriptsize{(MICCAI'21)} &7  &28     &61.55 &- &- &9.63 \\
    CPS~\cite{chen2021semi}\dag \scriptsize{(CVPR'21) }&7  &28      &78.40  &65.59  &5.88  &\textbf{1.55} \\
    SALCC~\cite{liu2022semi} \scriptsize{(MICCAI'22)}  &7  &28      &70.30  &-  &-  & 4.69\\
    MC-Net$+$~\cite{wu2022mutual}\dag \scriptsize{(MIA'22)} &7  &28      &66.91  &55.26  &12.74  &2.41 \\
    Ours &7  &28        &\textbf{83.10} &\textbf{71.79} &\textbf{4.76} &1.86 \\
    \hline
  \end{tabular} 
  % }
\end{table*}

==> table/Pancreas-CT.tex <==
\begin{table*}
  \centering
  \caption{Quantitative segmentation results on the Pancreas-CT dataset~\cite{clark2013cancer}. ~\dag~represents the reproduced results based on the open-sourced implementation.}
  \label{table:resluts on Pancreas-CT}
  % \setlength{\tabcolsep}{1mm}
    % \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c}{\#Scans used} &\multicolumn{4}{c}{Metrics} \\
    \cline{2-3} \cline{4-7} 
    &Labeled &Unlabeled &Dice(\%)$\uparrow$ &Jaccard(\%)$\uparrow$ &95HD$\downarrow$ &ASD$\downarrow$ \\
    \hline
    V-Net\dag &62  &0 &82.68 &71.05 &5.19 &1.41 \\
    \hline
    V-Net\dag &6  &0 &68.69 &55.03 &13.47 &3.63 \\
    % UA-MT~\cite{yu2019uncertainty}\scriptsize{(MICCAI'19)} &6  &56  &66.44 &52.02 &17.04 &3.03\\
    URPC~\cite{luo2021efficient} \scriptsize{(MICCAI'21)} &6  &56  &73.53 &59.44 &22.57 &7.85\\
    DTC\cite{luo2021semi} \scriptsize{(AAAI'21)} &6  &56  &66.58 &51.79  &15.46  &4.16 \\
    CPS~\cite{chen2021semi}\dag \scriptsize{(CVPR'21)} &6  &56  &73.16  &58.81  &15.67  &5.35 \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &6  &56 &74.01 &60.02 &12.59 &3.34\\
    Ours &6  &56 &\textbf{81.06} &\textbf{68.44} &\textbf{8.05} &\textbf{2.18} \\
    \hline
    V-Net\dag &12  &0  & 76.91 &63.86  &8.16  &2.07 \\
    % UA-MT~\cite{yu2019uncertainty}\scriptsize{(MICCAI'19)} &12  &50  &76.10 &62.62 &10.84 &2.43\\
    URPC~\cite{luo2021efficient} \scriptsize{(MICCAI'21)} &12 &50  &80.02 &67.30 &8.51 &1.98 \\
    DTC\cite{luo2021semi} \scriptsize{(AAAI'21)} &12 &50  &76.27  &62.82  &8.70  &2.20 \\
    CPS\cite{chen2021semi}\dag \scriptsize{(CVPR'21)} &12 &50  &79.46  &66.49  &10.34  &3.08 \\
    CVRL\cite{you2022momentum} \scriptsize{(MICCAI'22)} &12 &50      &76.68   &61.16  &8.24  &3.19 \\
    SimCVD \cite{you2022simcvd} \scriptsize{(TMI'22)}  &12 &50      &75.39   &61.56  &9.84 &2.33 \\
    MC-Net$+$~\cite{wu2022mutual} \scriptsize{(MIA'22)} &12 &50 &80.59 &68.08 &\textbf{6.47} &\textbf{1.74}\\
    Ours &12 &50 &\textbf{82.52} &\textbf{70.54} &7.11 &1.75 \\
    \hline
  \end{tabular}
  % }
\end{table*}

